Bayesian Incremental Learning for Deep Neural Networks

In industrial machine learning pipelines, data often arrive in parts. Particularly in the case of deep neural networks, it may be too expensive to train the model from scratch each time, so one would rather use a previously learned model and the new data to improve performance. However, deep neural networks are prone to getting stuck in a suboptimal solution when trained on only new data as compared to the full dataset. Our work focuses on a continuous learning setup where the task is always the same and new parts of data arrive sequentially. We apply a Bayesian approach to update the posterior approximation with each new piece of data and find this method to outperform the traditional approach in our experiments.

==> content/img/mnist+cifar10.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{icml2018_inc/content/img/mnist.png}
    \includegraphics[width=0.7\textwidth]{icml2018_inc/content/img/cifar10.png}
    \caption{Comparison of the conventional fine-tuning and the proposed Bayesian incremental learning approach on the LeNet5 and 3Conv3FC architectures on MNIST and CIFAR-10 datasets. The accuracy is reported for different posterior approximations for the training on the full dataset ($k$=$1$) and for the incremental learning of the dataset divided into $k$=$10$ parts. All reported accuracy is measured on the testing set. The experiment demonstrates that a more flexible posterior approximation allows us to perform more accurate variational inference and increase the quality of the final models.}
    \label{pic:mnistil}
    \label{pic:cifaril}
\end{figure}

==> content/img/pretraining.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\textwidth]{icml2018_inc/content/img/cifar5+5.png}
    \caption{
        Bayesian Incremental Learning results for pretrained (marked with~``-P'') and non-pretrained networks on the CIFAR(5+5) task. Laplace prior initialized pretrained network marked with~``-PL''.Reported accuracy values are measured on the subset of the test set which consists of objects of 5 classes corresponing to the second stage of CIFAR(5+5) experiment.  Second part of the training dataset divided into $k=10$ parts. Accuracies of models trained on the full second data part are reported as well ($k=1$).}
    \label{pic:cifar5+5}
\end{figure}
